Coordination Complexity: Small Information Coordinating Large Populations

We initiate the study of a quantity that we call coordination complexity. In a distributed optimization problem, the information defining a problem instance is distributed among $n$ parties, who need to each choose an action, which jointly will form a solution to the optimization problem. The coordination complexity represents the minimal amount of information that a centralized coordinator, who has full knowledge of the problem instance, needs to broadcast in order to coordinate the $n$ parties to play a nearly optimal solution. We show that upper bounds on the coordination complexity of a problem imply the existence of good jointly differentially private algorithms for solving that problem, which in turn are known to upper bound the price of anarchy in certain games with dynamically changing populations. We show several results. We fully characterize the coordination complexity for the problem of computing a many-to-one matching in a bipartite graph by giving almost matching lower and upper bounds.Our upper bound in fact extends much more generally, to the problem of solving a linearly separable convex program. We also give a different upper bound technique, which we use to bound the coordination complexity of coordinating a Nash equilibrium in a routing game, and of computing a stable matching.

==> Makefile <==
TOP=billboard
SRC= billboard lowerbound convex counter prelim intro stable privacy flowproof lower-proof
FLAGS=tex.flags
BIB=refs

.PHONY : clean
.PHONY : all
.PHONY : ps
.PHONY : long
.PHONY : short
.PHONY : comments

all: $(TOP).pdf $(FLAGS)

ps: $(TOP).ps

long: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fulltrue \\draftfalse' > ${FLAGS}
	@make

short: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fullfalse \\draftfalse' > ${FLAGS}
	@make

comments: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fulltrue \\drafttrue' > ${FLAGS}
	@make

%.pdf: $(SRC:=.tex) $(BIB).bib
	latexmk -pdf $<
	latexmk -c

%.ps : %.tex $(BIB).bib
	latexmk -ps $<
	latexmk -c

clean:
	latexmk -C


==> notes.tex <==
\section{Discussion Notes}
Consider a game of incomplete information with $n$ players along with
a mediator $\cM$ that has full knowledge of the underlying types of
the players. The mediator needs to coordinate the players to play
certain actions (for example, a Nash equilibrium) by broadcasting a
message on a \emph{billboard}. We develop a theory
of~\emph{coordination complexity}, where the central question to study
is the number of bits needed in the billboard message in order to
successfully coordinate the players.

We first give an obvious upper bound on the coordination complexity.
\begin{lemma}
Suppose the target action profile requires a description length of no
more than $m$ bits, then the mediator could coordinate the players to
play such joint actions with a billboard message of no more than $m$
bits.
\end{lemma}




\subsection{From Blackboard to Billboard: Relation to Communication Complexity}
Consider a multiparty communication model, in which $n$ players need
to compute a joint function of their data. The players can communicate
under the blackboard model -- each message sent by the players is
written on the billboard visible to all players. We first show that
blackboard communication complexity gives an upper bound on the
billboard coordination complexity.

\begin{lemma}
Suppose that there exists a protocol such that it requires at most $m$
bits of communication messages on the blackboard to compute some
action profiles for the players. Then there also exists a mediator
that uses at most $m$ bits of billboard messages to coordinate the
players to play the same action profile.
\end{lemma}

\begin{proof}
The mediator can simply post on the billboard the history of the
blackboard messages based on the protocol.
\end{proof}


\begin{table}[h]
\centering
    \begin{tabular}{|p{4cm}|p{5cm}|p{5  cm}|} \hline
    ~                             & High Coordination Complexity & Low Coordination Complexity \\ \hline
    High Communication Complexity & Proposed problem: Each player is has a binary bit $b_i$ and also a $n$-bit vector $Q_i$, and is interested to know $b\oplus Q_i$                            & Computing Parity                           \\\hline
    Low Communication Complexity  & ~                            & Computing average (or any computation that allows sub-sampling)                           \\\hline
    \end{tabular}
\end{table}


\subsection{Interface with Privacy}
Consider the analyst privacy problem: each of the $n$ analysts is
interested in answering a counting query on some underlying database
defined by the private data of the analysts.

Suppose that privacy of the analyst is not a constraint. Then we will
be able to answer all of the queries with accuracy $\alpha$ by
broadcasting a small database of size $\frac{\log n}{\alpha^2}$.

Now suppose the mediator wants to release the answers via a
$\eps$-differentially private billboard message. We can argue that
this message could hardly be useful. By the guarantee of differential
privacy, the probability distribution over the possible messages
remain about the same even if an analyst switches to a different
query. Then a good accuracy guarantee of the billboard message implies
that it could answer any other query with high accuracy as well (with
high probability). This contradicts with the privacy constraint.

We could circumvent this issue by introducing shared randomness
between the mediator and each player. Suppose that each player also
submits a random string to the mediator along with their types. Then
the mediator could simply post-process the answer to each player's
query by taking the XOR between her random string and query
answer. Posting post-processed answers on the billboard will not
compromise the analysts' privacy. (This is equivalent to the mediator
whispering to each analyst their query answer).


Note that the billboard message now has to scale with $n$, as opposed
to $\log n/\alpha^2$ in the non-private scenario. We will interested
in characterize problems that requires only sublinear bits on the
billboard message.


\subsection{Discussion on July 3rd}


\begin{itemize}
\item We need an example that separates communication complexity and coordination
complexity. One example would be the many-to-one matching.

\item The relation between JDP and coordination complexity. Suppose that a problem is low-sensitive
and has low coordination complexity. Then one could just implement the
exponential mechanism to select the approximately welfare maximizing
coordination strings. This gives an additive approximation of
$O(m/\eps)$.

\item Rounding in the convex programming approach cannot get arbitrarily small approximation.

\item The billboard type of algorithm might imply low coordination complexity in the same problem
maybe ($\eps n$).

\item Noisy counter approach allows us to get upper bound for other problems: routing and
stable matching.

\end{itemize}



==> templowerbound.tex <==
\section{Lower Bounds for Bipartite Matching}
In this section, we present lower bounds on the coordination
complexity of bipartite matching problems. As a building block, we
prove a lower bound for the one-to-one matching problem on a bipartite
graph with $n$ vertices on each side, showing an $\Omega(n)$ lower
bound -- i.e. that no substantial improvement on the trivial solution
is possible. We then extend this lower bound to the problem of
many-to-one matchings, in which there are $n$ agents who must be
matched to $k$ goods (each good can be matched to many agents, up to
its supply). Here, we show an $\Omega(k)$ lower bound. In the next
section, we give a nearly matching upper bound, which substantially
improves over the trivial solution.


\subsection{A Variant of the Index Function Problem}
Before we present our lower bound, we introduce a variant
of the~\emph{random index function} problem~\cite{KNR99},\sw{maybe cite
  others too} that will be useful for our proof.

\paragraph{MULTIPLE-INDEX}{
There are two players Alice and Bob. Alice receives as input a
sequence of $t$ pairs, $I=\langle (S_i, u_i): i = 1,2, \ldots, t
\rangle$, where the $S_i$ are disjoint sets each with $k$ elements,
and $u_i$ is uniformly distributed in $S_i$. Based on her input Alice
sends Bob a message $M(I)$.  Bob then receives $(S_j,j)$, where $j$ is
chosen from $[t]$. Bob must determine $u_j$; let his output be
$B(S_j,j, M(I)) \in S_j$. We say that the protocol succeeds if $B(S_j,j,
M(I))=u_j$.  Let $\ell(t,k,p)$ be the minimum number of bits (for the
worst input) that Alice must send in order for Bob to succeed with
probability at least $p$.}

\ar{This part needs to be formalized a bit} 

Note that if Bob guesses randomly, then the protocol already succeeds
with probability $p = 1/k$. The following result shows that any
significant improvement over this trivial probability of success will
require Alice to send Bob a long message.

\begin{lemma}\label{index}
For $p \geq 1/k$, we have $\ell(t,k,p) \geq (8\log e) t(p - 1/k)^2$.
\end{lemma}
\ar{Needs to be formalized. For any protocol with success probability at least ..., the length of the message must be... Actually, can this just be stated as a communication complexity lower bound? I guess then we might need to define communication complexity..}
\jr{I have tried to make the definitions more formal.}


\begin{proof}
%% Fix the sequence of sets $S_1, S_2, \ldots , S_t$, each with $k$
%% elements. Consider the sequence of random variables
%% \[
%% W = (W_1, W_2, \ldots , W_t),
%% \]
%% which correspond to the set of $t$ special elements in the sets, and
%% each $W_i$ is chosen uniformly at random from $S_i$.
Fix a protocol where the coordinator broadcasts $\ell$ bits in the worst 
case. We will show that $\ell$ must be large.
Let $M(I)$ be the (random) message that Alice sends to Bob based on
her input $I$. Let $S(I) = \langle S_1, S_2, \ldots, S_t \rangle$ and
$u(I)=\langle u_1,u_2,\ldots,u_t \rangle$.  Then, $S(I)$, $u(I)$ and
$M(I)$ are random variables. Fix a value $S$ for $S(I)$ and so that
conditioned on ``$S(I)=S$'' the the probability of success is at least
$p$ (such an $S$ must exist). Then,
\[
I[u(I) :  M(I)] = H[M(I)  - H(M(I) \mid u(I)) \leq H(M(I)) \leq \Expectation[|M(I)|]
\leq \ell.
\]
On the other hand, since $u_1, u_2, \ldots, u_t$ are independent (conditioned
on ``$S(I)=S$''), we have
\[
\ell \geq I[u(I) : M(I)] \geq I[u_1 : M(I)] + \cdots + I[u_t : M(I)],
\]
implying that
\[
\Expectation_{i} \left[  I[u_i : M(I)]\right] \leq \frac{\ell}{t}.
\]
Let $u_{iz}$ denote the random variable whose distribution is the same
as that of $u_i$ when conditioned on the event $M(I)=z$, and let the
distance between the distributions of $u_{iz}$ and $u_i$ be
\[ \delta(u_{iz}, u_i) := \sum_{w \in S_i} |\Pr[u_{iz}=w] -\Pr[u_i=w]|.\]
Then, we have
\begin{align*}
I[u_i : M(I)] =& \Expectation_z \left[\KL(u_{iz} : u_i) \right] & \mbox{(from definition)}\\
\geq & (2 \log e) \Expectation_z \left[\left(\delta(u_{iz}, u_i)\right)^2 \right] & \mbox{(by Pinsker's inequality)} \\
\geq & (2\log e) \left(\Expectation_z\left[\delta(u_{iz} , u_i) \right]\right)^2.
& \mbox{(by Jensen's inequality)}
\end{align*}
With one more
application of Jensen's inequality, we obtain the following
\[
\Expectation_{i} \left[I[u_i : M(I)]\right] \geq
(2\log e) \Expectation_{i} \left[ \left(\Expectation_z\left[\delta(u_{iz} : u_i)
    \right] \right)^2 \right] \geq
(2\log e) \left(\Expectation_{i} \left[ \Expectation_z\left[\delta(u_{iz} : u_i)
    \right] \right]\right)^2.
\]
Suppose Bob succeeds in guessing the special element of $S_i$ with
probability $p_i$; then $\Expectation_i[p_i] = p$. 
Furthermore, we have $\delta(u_{iz}, u_i) \geq
2|p_i- 1/k|$. Thus, by Jensen's inequality, we have
\[
\left(\Expectation_{i} \left[ \Expectation_z\left[\delta(u_{iz} : u_i)
    \right] \right]\right)^2 \geq 4(p - 1/k)^2
\]
It follows that $\ell /t \geq (8\log e) (p-1/k)^2$, that is, $\ell
\geq (8 \log e) t(p-1/k)^2$.
\end{proof}


\subsection{Lower Bound for One-to-One Matchings}\label{sec:1to1}
We will first focus on the lower bound on one-to-one matching and show
the following.
\begin{theorem}\label{1to1}
Suppose the coordination protocol $\Pi$ for one-to-one matching
guarantees an approximation ratio of $\rho$ in expectation. Then, the
coordinator of $\Pi$ must broadcast $\Omega(n/\rho^4)$ bits on problem
instances of size $n$ (in the worst case).
\end{theorem}

Fix the protocol $\Pi$. We will extract a two-party communication
protocol for the MULTIPLE-INDEX problem from $\Pi$, and use the above
lemma. As a first step for our lower bound proof, we will consider the
following random graph construction process $\ranG$.

\paragraph{Random Graph Construction $\ranG(\rho, n)$:}{
Let $a = (1/16) n/\rho^2$ and $k = 2\rho$. Consider the following
random bipartite graph $G$ with vertex set $(V, W)$ such that $|V| =
|W| = n$.
\begin{itemize}
\item Randomly generate an ordering $w_1,w_2, \ldots, w_n$ of $W$ (all
  $n!$ orderings being equally likely), and partition $W$ as
  $W_1 \cup W_2$ such that $W_1=\{w_1,w_2,\ldots,
  w_{ak}\}$, and $W_2=\{w_{ak+1}, w_{ak+2}, \ldots, w_n\}$.

\item Similarly, randomly generate an ordering $v_1, v_2, \ldots, v_n$
  of $V$, and parition $V$ into $n/a$ bocks, $B_1, B_2, \ldots, B_{n/a}$
  (each with $a$ vertices), where
\[ B_j := \{v_i: (j-1)a + 1  \leq i \leq ja\}.\]

\item Connect $B_j$ and $W$ as follows.  First, we describe the
  connections between $V$ and $W_1$.  The neighbourhoods of the
  vertices in each $B_j$ will be disjoint: we partition
  $W_1$ into equal-sized disjoint sets $(T_v: v \in B_j)$, and let the
  neighbours of $v \in B_j$ be exactly the $k$ vertices in $T_v$.


\item In addition, assign each vertex in $v$ one neighbor in $W_2$, by
  connecting $V$ with $W_2$ in round-robin fashion: so, vertex
  $v_i$ is connected to vertex $w_j$, where $j= \left(ak+1 + (i-1)
  \mod (n-ak)\right)$.  \jr{I have changed the expression; I hope I
    have not messed it up.}
\end{itemize}
}

Let us first observe that a graph generated by $\ranG$ always has a
matching with high welfare.

\begin{lemma}
 Each graph $G$ generated by the above process $\ranG(\cdot, n)$
 admits a matching with cardinality at least $\frac{7n}{8}$, that is,
 for each such graph $G$, the welfare objective satisfies $\OPT(G)
 \geq \frac{7n}{8}$.  
\ar{Have we defined ``The welfare objective''?}
\end{lemma}

\begin{proof}
\iffalse
  The proof follows from a simple application of the Hall's
  theorem. Fix any subset $S\subseteq W$. Let $N\colon 2^W \rightarrow
  2^V$ denotes the neighborhood function that maps any subset of $W$
  to its neighbors in $V$. It suffices to show that $|S| \leq |N(S)|$.

  Let $S_1 = S\cap W_1$ and $S_2 = S\cap W_2$. Note by the
  construction specified in $\ranG$, each vertex in $S_1$ is connected
  to $(n/a)$ distinct vertices in $V$ (one from each block $B_j$), and
  each vertex in $S_2$ is connected to at least 1 distinct vertex in
  $V$ \fi

Given the fixed ordering over the vertices in $V$, match each of its
first $(1 - \frac{1}{8\rho})n$ vertices to its unique neighbor in
$W_2$. Since $\rho\geq 1$, this gives a matching with welfare at
least
\[
\left(1 - \frac{1}{8\rho}\right) n \geq \frac{7n}{8},
\]
justifying our claim.
\end{proof}

We will now proceed to prove~\Cref{1to1}.

\begin{proof}[Proof of~\Cref{1to1}]
Let $\Pi$ be a coordination protocol with coordination complexity
$\ell$ and approximation ratio $\rho$. This means that on a graph
instance generated by $\ranG(\cdot, n)$, the parties can coordinate on
\jr{I don't understand $\ranG(\codt,n)$.}  a matching with expected
weight at least $\frac{7n}{8\rho}$.  Since $|W_1| = \frac{n}{8\rho}$,
we know in expectation at least $\frac{7n}{8\rho} - \frac{n}{8\rho} =
\frac{3n}{4\rho}$ of the vertices in $W_2$ are matched. Let $\alpha_v$
be the probability that in $\Pi$, agent $v$ picks her neighbor in
$W_2$. Then, by linearity of expectation, $\sum_{v \in V} \alpha_v
\geq \frac{3n}{4}$, that is, $\Expectation_{v \in V}[\alpha_v] \geq
\frac{3}{4}$.  Hence, there must be some block $B_j$ such that
$\Expectation_{v \in B_j}[\alpha_v] \geq \frac{3}{4}$. We will now
restrict attention to the block $B_j$ and consider the following
instance of {\bf MULTIPLE-INDEX}: for each $v\in B_j$, set $S_v =
N(v)$---the neighborhood of vertex $v$, and let $u_v$ be the vertex
unique vertex in $S_v\cap W_2$. Since the message broadcast by the
coordination protocol allows the players to identify the special
element with average success probability of $\frac{3}{4\rho}$,
by~\Cref{index} the length of message
\begin{align*}
\ell & \geq (8\log e) |B_j| \left(\frac{3}{4\rho} - \frac{1}{k}\right)\\
     & \geq (8 \log e) a \left(\frac{3}{4\rho} - \frac{1}{2\rho}\right)\\
&\geq (8 \log e) \left(\frac{n}{16\rho^2}\right) \left( \frac{3}{4\rho} -
\frac{1}{2\rho + 1} \right)^2\\
& \geq \frac{n}{32\rho^4},
\end{align*}
which completes the proof.
\end{proof}


\subsection{Lower Bound for Many-to-One Matchings}
Finally, we give the following lower bound on coordination complexity
for many-to-one matchings. The lower bound relies on the result
from~\Cref{sec:1to1}---we show that any coordination protocol for
many-to-one matchings can also be reduced to a protocol for one-to-one
matchings, and so the lower bound in~\Cref{sec:1to1} can be extended
to give a lower bound for the many-to-one setting.

Recall that in a many-to-one matching problem, there is a bipartite
graph $G = (V, E)$ such that the vertices in $V$ represent $n$
different players and $W$ represent a set of $k$ goods $j$, each with
a supply $s_j$.

\jr{Should we say that in our lower bound instance, all $s_j=b$?}

\begin{theorem}\label{thm:many-to-one}
Suppose that there exists a coordination protocol for many-to-one
matchings that guarantees an approximation ratio of $\rho$ in
expectation. Then such a protocol has coordination complexity of
$\Omega(k / \rho^{4})$.
\end{theorem}

We will start by considering a one-to-one matching instance with $k$
vertices on each side of the graph $G' = (V', W', E')$. Suppose that
this graph has an optimal matching of size $\OPT'$. In order to match
the lower bound result in one-to-one matchings, we assume that $\OPT'
\geq \frac{7k}{8}$. \ar{Shouldn't we just assume that the $k\times k$
  one-to-one matching instance is generated by the process that
  generated the lower bound instance in the section above?}

\jr{I agree. Let us just say that we start with the $k \times k$ instance
from the section above.}

Now we will turn this into an instance of a many-to-one matching
problem: make $b$ copies of each vertex in $V'$ to obtain vertex set
$V$, and set $W:= W'$, with the supply of good $j$ as $s_j =
b$; then for an edge $(v', w')$ in the original graph, connect all
copies of $v'$ to $w'$ in the new graph. This gives a bipartite graph
$G = (V, W, E)$. The following claim is straightforward.
\begin{claim}
The new graph $G$ has a matching of size at least $(b\OPT')$.
\end{claim}

Now suppose that we could coordinate the players in $V$ to obtain a
matching $M^*$ of size $\frac{b\OPT'}{\rho}$ in $G$. Then with a simple
sampling procedure, we can extract a high cardinality matching for
the original graph: for each vertex in $v' \in V'$, sample one of the
$b$ copies of $v'$ in $G$ uniformly at random along with its incident
matched edge. If two vertices in $V'$ are connected to the same type
of good in $W'$, break ties arbitrarily and keep only one of the
edges.

\begin{lemma}\label{goodwelfare}
  The sampled matching in $G'$ has expected size at least
  $\frac{\OPT'}{3\rho}$.
\end{lemma}

\begin{proof}
For $w \in W'$, let $d_w$ be the number of copies of good $w$ that
have been assigned in the matching $M^*$. Then $\sum_w d_w \geq
b\OPT'/\rho$.  If $d_w \geq 1$, then we have the following
estimate for the probability that $w$ is chosen.
\begin{align}
\Pr[\mbox{$w$ is chosen}]
&\geq d_w \frac{1}{b} \left(1 - \frac{1}{b}\right)^{d_w -1}\\
&\geq \frac{d_w}{b} \left(1 + \frac{1}{b-1}\right)^{-(d_w -1)}\\
&\geq \frac{d_w}{b} \exp(-(d_w-1)/(b-1)) & \mbox{because $1+x \leq e^x$}\\
&\geq \frac{d_w}{eb}. & \mbox{(because $d_w \leq b$)}.
\end{align}
In particular, by linearity of expectation
\[
\Expectation[|M^*|]  \geq \sum_{w \in W'} \frac{d_w}{eb}\\
\geq \frac{b \OPT'}{e b \rho} \geq \frac{\OPT'}{3\rho}.
\]
\end{proof}

\jr{I have tried to avoid some applications of Markov's
  inequality. Please check}

\iffalse
\begin{proof}[The old proof.]
Let $\mu \subseteq E$ be the matching the players coordinate on in
$G$. To simplify our analysis, we will first discard all of
the goods that contribute less than $\frac{b}{2\rho}$ to the total welfare. We
will first bound the loss of welfare due to this process. Suppose that
there are a $\gamma$ fraction of the $k$ types of goods that are
discarded.  Since on average each type of good is incident to
$\frac{b\OPT'}{k\rho}$ edges, we have
\[
\gamma \frac{b}{2\rho} + (1 - \gamma) b \geq \frac{b\OPT'}{m\rho}
\]
\ar{What is $m$?} which means
\[
 \gamma \leq \frac{2\left(\rho - \OPT'/k \right)}{2\rho - 1}.
\]
Then the remaining graph $G$ should still have a matching of size at
least
\[
R = \left(\frac{\frac{2\OPT'}{k} - 1}{2\rho - 1}\right)\left( \frac{b
  \OPT'}{\rho}\right).
\]
Now apply the sampling step to $G$ and sample a copy of each vertex
$v' \in V'$ uniformly at random. Note that each of the remaining goods
has at least $q = \frac{b}{2\rho}$ incident edges in $G$, and contributes 
welfare 1 in the sampled matching whenever at least 1 sampled agent is matched to it.

For each of the goods, the chance that it has exactly 1 person matched
to it is:
\[
q \left(\frac{1}{b}\right) \left(\frac{b-1}{b} \right)^{(q-1)} \approx
\frac{q}{b} \cdot (1/e)^{(q-1)/b} \geq \Omega\left(\frac{1}{\rho}\right)
\]
\ar{Approximately $\approx$ ???} Therefore, the sample matching has a welfare of at least
\[
\Omega\left( \frac{R}{\rho b}\right) = \Omega\left( \frac{\OPT'}{\rho^3}\right)
\]
which recovers the stated bound.
\end{proof}
\fi

We now have all the pieces to prove~\Cref{thm:many-to-one}.
\begin{proof}[Proof of~\Cref{thm:many-to-one}]
Suppose that there exists a coordination protocol $(\sigma, \pi)$ for
many-to-one matchings with a guaranteed approximation ratio of
$\rho$. By~\Cref{goodwelfare}, 

By the result of~\Cref{goodwelfare}, we know that this coordination
protocol for one-to-one matchings has an approximation ratio 
most $O(\rho)$. By the lower bound in~\Cref{1to1}, we know that the
length of $\sigma(G)$ is at least $\Omega(k/\rho^{4})$.

\iffalse
We can turn this into coordination protocol for one-to-one
matchings: given any bipartite graph $G'$, make $b$ copies of each
node in $G'$ to obtain a new graph $G$; the coordinator broadcasts
message $\sigma(G)$; each player $v'$ in the original graph $G'$ will
then be able to compute the sub-matching $\mu_{v'}$ restricted the $b$
copies of $v'$ based on the decode function $\pi$ and the message
$\sigma(G)$; lastly, each player $v'$ sample an edge from the
$\mu_{v'}$ as its edge.

By the result of~\Cref{goodwelfare}, we know that this coordination
protocol for one-to-one matchings has an approximation ratio of at
most $\rho^3$. By the lower bound in~\Cref{1to1}, we know that the
length of $\sigma(G)$ is at least $\Omega(k/\rho^{12})$.
\fi
\end{proof}




























\iffalse
\subsection{Lower Bound for Matching}
We will show the following lower bound on the coordination complexity.
Let $\OPT(G)$ denote the size of the maximum matching for the
underlying graph $G$, and given any signaling scheme $\sigma$ and
matching protocol $\Pi$, let the performance ratio be $\rho = \OPT(G)
/ value(G, \sigma, \Pi)$.


\begin{theorem}
Suppose that the performance ratio at most $\rho$. Then the message
published by the coordinator has length
\[
m \geq \Omega(n/\rho^4).
\]
\end{theorem}
\fi

